{\mu}Touch: Enabling Accurate, Lightweight Self-Touch Sensing with Passive Magnets

Self-touch gestures (e.g., nuanced facial touches and subtle finger scratches) provide rich insights into human behaviors, from hygiene practices to health monitoring. However, existing approaches fall short in detecting such micro gestures due to their diverse movement patterns. This paper presents {\mu}Touch, a novel magnetic sensing platform for self-touch gesture recognition. {\mu}Touch features (1) a compact hardware design with low-power magnetometers and magnetic silicon, (2) a lightweight semi-supervised framework requiring minimal user data, and (3) an ambient field detection module to mitigate environmental interference. We evaluated {\mu}Touch in two representative applications in user studies with 11 and 12 participants. {\mu}Touch only requires three-second fine-tuning data for each gesture, and new users need less than one minute before starting to use the system. {\mu}Touch can distinguish eight different face-touching behaviors with an average accuracy of 93.41%, and reliably detect body-scratch behaviors with an average accuracy of 94.63%. {\mu}Touch demonstrates accurate and robust sensing performance even after a month, showcasing its potential as a practical tool for hygiene monitoring and dermatological health applications. Code is available at https://wangmerlyn.github.io/muTouch/.

==> figures/pipeline/pipeline_figure.tex <==
\definecolor{darkbrown}{rgb}{0.4, 0.26, 0.13}
\definecolor{darkbyzantium}{rgb}{0.36, 0.22, 0.33}
\definecolor{darkcandyapplered}{rgb}{0.64, 0.0, 0.0}
\definecolor{darkcerulean}{rgb}{0.03, 0.27, 0.49}
\definecolor{darkchampagne}{rgb}{0.76, 0.7, 0.5}
\definecolor{darkchestnut}{rgb}{0.6, 0.41, 0.38}
\definecolor{darkcoral}{rgb}{0.8, 0.36, 0.27}
\definecolor{darkcyan}{rgb}{0.0, 0.55, 0.55}
\definecolor{darkslategray}{rgb}{0.18, 0.31, 0.31}
\definecolor{cadetblue}{rgb}{0.37, 0.62, 0.63}
\definecolor{darklavender}{rgb}{0.45, 0.31, 0.59}
\definecolor{mauvetaupe}{rgb}{0.57, 0.37, 0.43}
\definecolor{russet}{rgb}{0.5, 0.27, 0.11}
\tikzstyle{annot} = [text width=4em, text centered]
\tikzstyle{arrow} = [thick,->,>=latex]
\definecolor{pltred}{HTML}{831D2B}
\definecolor{pltcyn}{HTML}{3F88C5}
\definecolor{pltbrn}{HTML}{C7985B}

\definecolor{brightlavender}{rgb}{0.75, 0.58, 0.89}
\definecolor{burntorange}{rgb}{0.8, 0.33, 0.0}
\definecolor{celadon}{rgb}{0.67, 0.88, 0.69}
\definecolor{darkturquoise}{rgb}{0.0, 0.81, 0.82}
\definecolor{dodgerblue}{rgb}{0.12, 0.56, 1.0}	
\definecolor{firebrick}{rgb}{0.7, 0.13, 0.13}
\definecolor{limegreen}{rgb}{0.2, 0.8, 0.2}
\definecolor{green(munsell)}{rgb}{0.0, 0.66, 0.47}
\definecolor{mayablue}{rgb}{0.45, 0.76, 0.98}
\definecolor{mediumaquamarine}{rgb}{0.4, 0.8, 0.67}
\usetikzlibrary{patterns} % LATEX and plain TEX when using TikZ
\usetikzlibrary[patterns] % ConTEXt when using TikZ
\usetikzlibrary{decorations.pathreplacing, calligraphy}
\usetikzlibrary {arrows.meta}

\begin{figure}[H]
\begin{tikzpicture}

\node[] at (-0.3, -1.1) {\includegraphics[width = 0.07\textwidth]{figures/encoder2.png}};
\node[] at (-0.3, -2.6){\includegraphics[width=0.08\textwidth]{figures/pipeline/svmlogo2.png}};


% \draw[->] (0, 0) --(6.6, 0);
% \draw[->] (0, 0) --(0, 2.5);
% \draw[thick]  plot [smooth,tension=0.8] coordinates {(0, 0) (0.5, 0.35) (1.0, 1.66) (1.5, 1.21) (2.0, 1.76) (2.5, 1.35) (3.0, 2.25) (3.5, 1.34) (4.0, 2.02) (4.5, 1.11) (5.0, 1.65) (5.5, 0.68) (6.0, 0.2) (6.25, 0.05) (6.5, 0)};
\draw[->] (0, 0) --(8.6, 0);
\draw[->] (0, 0) --(0, 3.2);
\node[font = \large] at (0.8, 3.4) {Magnetic Field Readings};
\node[font = \Large] at (8.9, -0.35) {Time};
\draw[thick]  plot [smooth,tension=0.8] coordinates {(0, 0) (0.5, 0.55) (1.0, 1.76) (1.5, 1.16) (2.0, 2.32) (2.5, 1.71) (3.0, 2.65) (3.5, 2.04) (4.0, 2.72) (4.5, 1.94) (5.0, 2.35) (5.5, 1.78) (6.0, 2.21) (6.5, 1.72) (7.0, 1.89) (7.5, 0.85) (8.0, 0.25) (8.25, 0.08) (8.5, 0)};

% \def\sqrpos{1.85, 1.7, 1.95, 2.1, 2.35, 2.0, 2.2, 1.9, 1.86, 1.0}
\def\sqrpos{1.85/blue, 1.95/green, 2.48/blue, 2.56/blue, 2.8/blue, 2.95/blue, 2.7/grey, 2.57/cyan, 2.45/magenta, 2.35/red, 2.2/blue, 1.4/blue}
\def\sqheight{0.9}

\def\recheight{1.25}
\def\recwidth{0.5}
\def\recdist{0.6}
\def\xoffset{0.1}

\def\colorsold{
russet, cadetblue, cadetblue, 
darkcerulean, cadetblue, cadetblue, 
cadetblue, darkchampagne, cadetblue, 
cadetblue, darkcoral, russet}

\def\colors{
brightlavender, mayablue, mayablue,
limegreen, mayablue, mayablue, 
mayablue, firebrick, mayablue, 
mayablue, burntorange, brightlavender}

\foreach \cls [count = \x] in \colors {
    \fill[\cls, opacity = 0.6] (\x * \recdist + \xoffset, -0.5) rectangle ++(\recwidth, - \recheight);
}

\def\patterns{
crosshatch dots, north east lines, north east lines, 
north west lines,  north east lines, north east lines, 
north east lines, grid, north east lines, 
north east lines, horizontal lines, crosshatch dots}

\foreach \pts [count = \x] in \patterns {
    \draw[pattern = \pts] (\x * \recdist + \xoffset, -0.5) rectangle ++(\recwidth, - \recheight);
    % \draw[->, thick] (\x * \recdist + \xoffset + 0.5 * \recwidth, -0.6 - \recheight) -- (\x * \recdist + \xoffset + 0.5*\recwidth + \x*0.02 - 0.02*5.5, -1.1 - \recheight);
}
\foreach \sqp/\cls [count = \x] in \sqrpos {
    \draw[draw = red!40!black, thick, opacity = 0.7] (\x * \recdist + \xoffset - 0.1, \sqp) rectangle ++(\recwidth + 0.2, - \sqheight);
    \draw[->, thick] (\x * \recdist + \xoffset + 0.5 * \recwidth, \sqp - \sqheight - 0.2) -- (\x * \recdist + \xoffset + 0.5*\recwidth, -0.4);
}

% \readlist*\patternlist{"horizontal lines", "vertical lines", "north east lines", "north west lines", "grid", "crosshatch", "crosshatch dots"}
% \readlist*\patternchoice{1, 0, 0, 3, 0, 0, 2, 0, 5, 0, 3, 4, 0, 0, 0, 6}
% \readlist*\patterns{horizontal lines, vertical lines, vertical lines, north west lines,  "vertical lines", "vertical lines", "north east lines", "vertical lines",  "crosshatch", "vertical lines", "north west lines", "grid",  "vertical lines", "vertical lines", "vertical lines", "crosshatch dots"}
% \readlist*\patterns{horizontal lines, vertical lines, vertical lines, north west lines,  vertical lines, vertical lines, north east lines, vertical lines,  crosshatch, vertical lines, north west lines, grid,  vertical lines,  vertical lines, vertical lines, crosshatch dots}
% \setsepchar{,}

\def\answers{
no touching, left eye, left eye, 
right eye, left eye, left eye, 
left eye, forehead, left eye, 
left eye, left cheek, no touching}

\foreach \ans [count = \x] in \answers {
    % \node[font = \small, rotate = 45] at (\x*\recdist + \xoffset + 0.5*\recwidth + \x*0.02 - 0.02*5.5, -1.3 - \recheight) {\ans};
    \node[font = \small, rotate = 45] at (\x*\recdist + \xoffset + 0.5*\recwidth, -1.3 - \recheight) {\ans};
}

\node [] at (-0.3, -4.0) {Majority Vote};
\node [] at (6 * \recdist + 0.7, -4.0) {left eye};
\draw[decorate, decoration = {calligraphic brace, amplitude = 10pt}, thick] (8.25, -3.25) -- (0.25, -3.25);

\draw [line width=0.5pt, double distance=2pt, arrows = {-Latex[length=0pt 2 0]}] (0.1, -0.1) -- (-0.3, -0.65);
\draw [line width=0.5pt, double distance=2pt, arrows = {-Latex[length=0pt 2 0]}] (-0.3, -1.6) -- (-0.3, -2.05);
\draw [line width=0.5pt, double distance=2pt, arrows = {-Latex[length=0pt 2 0]}] (-0.3, -3.15) -- (-0.3, -3.7);

\end{tikzpicture}
\caption{The flowchart of the face touching detection inference pipeline.} 
\label{fig:face_touching_inference_pipeline}
\end{figure}

